A formalisation of XMAS

Communication fabrics play a key role in the correctness and performance of modern multi-core processors and systems-on-chip. To enable formal verification, a recent trend is to use high-level micro-architectural models to capture designers' intent about the communication and processing of messages. Intel proposed the xMAS language to support the formal definition of executable specifications of micro-architectures. We formalise the semantics of xMAS in ACL2. Our formalisation represents the computation of the values of all wires of a design. Our main function computes a set of possible routing targets for each message and whether a message can make progress according to the current network state. We prove several properties on the semantics, including termination, non-emptiness of routing, and correctness of progress conditions. Our current effort focuses on a basic subset of the entire xMAS language, which includes queues, functions, and switches.

==> eptcsdata.tex <==
\providecommand{\firstpage}{111}
\providecommand{\publicationstatus}{R. Gamboa and J. Davis (Eds.): ACL2 Workshop 2013 (ACL2 '13).\\
EPTCS 114, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.114.9}{10.4204/EPTCS.114.9}}
\pdfoutput=1

